Studying Scientific Data Lifecycle in On-demand Distributed Storage Caches

The XRootD system is used to transfer, store, and cache large datasets from high-energy physics (HEP). In this study we focus on its capability as distributed on-demand storage cache. Through exploring a large set of daily log files between 2020 and 2021, we seek to understand the data access patterns that might inform future cache design. Our study begins with a set of summary statistics regarding file read operations, file lifetimes, and file transfers. We observe that the number of read operations on each file remains nearly constant, while the average size of a read operation grows over time. Furthermore, files tend to have a consistent length of time during which they remain open and are in use. Based on this comprehensive study of the cache access statistics, we developed a cache simulator to explore the behavior of caches of different sizes. Within a certain size range, we find that increasing the XRootD cache size improves the cache hit rate, yielding faster overall file access. In particular, we find that increase the cache size from 40TB to 56TB could increase the hit rate from 0.62 to 0.89, which is a significant increase in cache effectiveness for modest cost.

==> Makefile <==
###############################################################################
# the latex command is pdflatex
LATEX = pdflatex -shell-escape
# the bibtex command is biber -- specified in preamble.tex in this directory
BIBTEX = bibtex

###############################################################################
# the main latex file 
MAIN = main

###############################################################################
# Assume all LaTeX files (*.tex) are in this level and all figures are in figs
# directory and all bibtex entries are at this level with .bib
TEXFILES = ${wildcard *.tex} ${wildcard */*.tex}
BIBFILES = ${wildcard *.bib}
FIGS = ${figs/wildcard *.pdf} ${figs/wildcard *.png} ${figs/wildcard *.jpg}

###############################################################################
# default target
.DEFAULT_GOAL := $(MAIN).pdf
$(MAIN): $(MAIN).pdf
.PHONY: $(MAIN) clean realclean

###############################################################################
# run LATEX command to generate the main PDF file
$(MAIN).pdf $(MAIN).log: $(TEXFILES) $(FIGS) $(BIBFILES)
	${LATEX} $(MAIN)
	@if [ `fgrep undefined $(MAIN).log | fgrep Citation - | wc -l` -gt 0 ]; then \
	${BIBTEX} $(MAIN); ${LATEX} $(MAIN); fi;
	@if [ `fgrep undefined $(MAIN).log | fgrep Citation - | wc -l` -gt 0 ]; then \
	${BIBTEX} $(MAIN); ${LATEX} $(MAIN); fi;
	@while [ `fgrep -i 'Rerun ' $(MAIN).log | fgrep LaTeX - | wc -l` -gt 0 ]; do \
        ${LATEX} $(MAIN); \
        done

###############################################################################
# basic sanity check
check: missingincludes badrefs badbibs

# Extract a list of missing smartinclude files
missingincludes: $(MAIN).log
	@(grep -i "smartinclude: warning:" $< | \
	  sed 's/smartinclude: WARNING: //' > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== SMARTINCLUDE WARNINGS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)

# Check log for: 
# - Multiply defined labels
# - Undefined labels
# - Undefined citations
# - Undefined acronyms (no messages for multiply-defined acronyms)
badrefs: $(MAIN).log
	@(grep -i "latex warning:" $< |\
	  grep -v -i "there were multiply-defined labels" | \
	  grep "multiply defined" |\
	  sed 's/LaTeX Warning: //' > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== MULTIPLY-DEFINED LABELS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "latex warning:" $< | \
	  grep -v -i "there were undefined references" | \
	  grep -i "reference" | grep -i "undefined" |\
	  sed 's/LaTeX Warning: //' > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== UNDEFINED LABELS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "package acronym warning:" $< | \
	  grep -i "acronym" | grep -i "not defined" |\
	  sed 's/Package acronym Warning: //' |\
	  sort | uniq > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== UNDEFINED ACRONYMS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)

# Check BibTeX log for:
# - missing .bib files
# - missing database entries
# - repeated entries
# - string name undefined
# - errors in entries ("I was expecting...")
badbibs: $(MAIN).log
	${BIBTEX} $(MAIN)
	@(grep -i "i couldn't open database file " $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== MISSING BIB FILES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "warning--i didn't find a database entry for" \
	  $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== MISSING BIB ENTRIES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "repeated entry--"  $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== REPEATED BIB ENTRIES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "warning--string name" $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== UNDEFINED STRINGS IN BIB =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "i was expecting"  $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== ERRORS IN BIB ENTRIES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)

clean:
	-@find . \( -name '*.aux' -print \) -o \( -name '*.log' -print \) \
		-o \( -name '*.bbl' -print \) -o \( -name '*.blg' -print \) \
		-o \( -name '*.toc' -print \) -o \( -name '*.out' -print \) \
		-o \( -name '*.bcf' -print \) -o \( -name '*~' -print \) \
		-o \( -name '*.maf' -print \) -o \( -name '*.mtc*' -print \) | xargs $(RM)

###############################################################################
# WARNING: removes the main target
realclean: clean
	$(RM) $(MAIN).pdf*

